Information Flow Analysis for a Dynamically Typed Functional Language with Staged Metaprogramming

Web applications written in JavaScript are regularly used for dealing with sensitive or personal data. Consequently, reasoning about their security properties has become an important problem, which is made very difficult by the highly dynamic nature of the language, particularly its support for runtime code generation. As a first step towards dealing with this, we propose to investigate security analyses for languages with more principled forms of dynamic code generation. To this end, we present a static information flow analysis for a dynamically typed functional language with prototype-based inheritance and staged metaprogramming. We prove its soundness, implement it and test it on various examples designed to show its relevance to proving security properties, such as noninterference, in JavaScript. To our knowledge, this is the first fully static information flow analysis for a language with staged metaprogramming, and the first formal soundness proof of a CFA-based information flow analysis for a functional programming language.

==> slamjs/coq-cfa/Makefile <==
#############################################################################
##  v      #                   The Coq Proof Assistant                     ##
## <O___,, #                INRIA - CNRS - LIX - LRI - PPS                 ##
##   \VV/  #                                                               ##
##    //   #  Makefile automagically generated by coq_makefile V8.3        ##
#############################################################################

# WARNING
#
# This Makefile has been automagically generated
# Edit at your own risks !
#
# END OF WARNING

#
# This Makefile was generated by the command line :
# coq_makefile cfa.v lambdajs.v lib.v simple_cfa.v 
#

# 
# This Makefile may take 3 arguments passed as environment variables:
#   - COQBIN to specify the directory where Coq binaries resides;
#   - CAMLBIN and CAMLP4BIN to give the path for the OCaml and Camlp4/5 binaries.
COQLIB:=$(shell $(COQBIN)coqtop -where | sed -e 's/\\/\\\\/g')
CAMLP4:="$(shell $(COQBIN)coqtop -config | awk -F = '/CAMLP4=/{print $$2}')"
ifndef CAMLP4BIN
  CAMLP4BIN:=$(CAMLBIN)
endif

CAMLP4LIB:=$(shell $(CAMLP4BIN)$(CAMLP4) -where)

##########################
#                        #
# Libraries definitions. #
#                        #
##########################

OCAMLLIBS:=-I .
COQSRCLIBS:=-I $(COQLIB)/kernel -I $(COQLIB)/lib \
  -I $(COQLIB)/library -I $(COQLIB)/parsing \
  -I $(COQLIB)/pretyping -I $(COQLIB)/interp \
  -I $(COQLIB)/proofs -I $(COQLIB)/tactics \
  -I $(COQLIB)/toplevel \
  -I $(COQLIB)/plugins/cc \
  -I $(COQLIB)/plugins/dp \
  -I $(COQLIB)/plugins/extraction \
  -I $(COQLIB)/plugins/field \
  -I $(COQLIB)/plugins/firstorder \
  -I $(COQLIB)/plugins/fourier \
  -I $(COQLIB)/plugins/funind \
  -I $(COQLIB)/plugins/groebner \
  -I $(COQLIB)/plugins/interface \
  -I $(COQLIB)/plugins/micromega \
  -I $(COQLIB)/plugins/nsatz \
  -I $(COQLIB)/plugins/omega \
  -I $(COQLIB)/plugins/quote \
  -I $(COQLIB)/plugins/ring \
  -I $(COQLIB)/plugins/romega \
  -I $(COQLIB)/plugins/rtauto \
  -I $(COQLIB)/plugins/setoid_ring \
  -I $(COQLIB)/plugins/subtac \
  -I $(COQLIB)/plugins/subtac/test \
  -I $(COQLIB)/plugins/syntax \
  -I $(COQLIB)/plugins/xml
COQLIBS:=-I . 
COQDOCLIBS:=

##########################
#                        #
# Variables definitions. #
#                        #
##########################

ZFLAGS=$(OCAMLLIBS) $(COQSRCLIBS) -I $(CAMLP4LIB)
OPT:=
COQFLAGS:=-q $(OPT) $(COQLIBS) $(OTHERFLAGS) $(COQ_XML)
ifdef CAMLBIN
  COQMKTOPFLAGS:=-camlbin $(CAMLBIN) -camlp4bin $(CAMLP4BIN)
endif
COQC:=$(COQBIN)coqc
COQDEP:=$(COQBIN)coqdep -c
GALLINA:=$(COQBIN)gallina
COQDOC:=$(COQBIN)coqdoc
COQMKTOP:=$(COQBIN)coqmktop
CAMLLIB:=$(shell $(CAMLBIN)ocamlc.opt -where)
CAMLC:=$(CAMLBIN)ocamlc.opt -c -rectypes
CAMLOPTC:=$(CAMLBIN)ocamlopt.opt -c -rectypes
CAMLLINK:=$(CAMLBIN)ocamlc.opt -rectypes
CAMLOPTLINK:=$(CAMLBIN)ocamlopt.opt -rectypes
GRAMMARS:=grammar.cma
CAMLP4EXTEND:=pa_extend.cmo pa_macro.cmo q_MLast.cmo
CAMLP4OPTIONS:=
PP:=-pp "$(CAMLP4BIN)$(CAMLP4)o -I $(CAMLLIB) -I . $(COQSRCLIBS) $(CAMLP4EXTEND) $(GRAMMARS) $(CAMLP4OPTIONS) -impl"

###################################
#                                 #
# Definition of the "all" target. #
#                                 #
###################################

VFILES:=cfa.v\
  lambdajs.v\
  lib.v\
  simple_cfa.v
VOFILES:=$(VFILES:.v=.vo)
VOFILES0:=$(filter-out ,$(VOFILES))
GLOBFILES:=$(VFILES:.v=.glob)
VIFILES:=$(VFILES:.v=.vi)
GFILES:=$(VFILES:.v=.g)
HTMLFILES:=$(VFILES:.v=.html)
GHTMLFILES:=$(VFILES:.v=.g.html)

all: $(VOFILES) 
spec: $(VIFILES)

gallina: $(GFILES)

html: $(VFILES)
	- mkdir -p html
	$(COQDOC) -utf8 -l -toc -html $(COQDOCLIBS) -d html $(VFILES)

gallinahtml: $(GLOBFILES) $(VFILES)
	- mkdir -p html
	$(COQDOC) -toc -html -g $(COQDOCLIBS) -d html $(VFILES)

all.ps: $(VFILES)
	$(COQDOC) -toc -ps $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.ps: $(VFILES)
	$(COQDOC) -toc -ps -g $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all.pdf: $(VFILES)
	$(COQDOC) -toc -pdf $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.pdf: $(VFILES)
	$(COQDOC) -toc -pdf -g $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`



####################
#                  #
# Special targets. #
#                  #
####################

.PHONY: all opt byte archclean clean install depend html

%.vo %.glob: %.v
	$(COQC) $(COQDEBUG) $(COQFLAGS) $*

%.vi: %.v
	$(COQC) -i $(COQDEBUG) $(COQFLAGS) $*

%.g: %.v
	$(GALLINA) $<

%.tex: %.v
	$(COQDOC) -latex $< -o $@

%.html: %.v %.glob
	$(COQDOC) -html $< -o $@

%.g.tex: %.v
	$(COQDOC) -latex -g $< -o $@

%.g.html: %.v %.glob
	$(COQDOC) -html -g $< -o $@

%.v.d: %.v
	$(COQDEP) -slash $(COQLIBS) "$<" > "$@" || ( RV=$$?; rm -f "$@"; exit $${RV} )

byte:
	$(MAKE) all "OPT:=-byte"

opt:
	$(MAKE) all "OPT:=-opt"

install:
	mkdir -p $(COQLIB)/user-contrib
	(for i in $(VOFILES0); do \
	 install -d `dirname $(COQLIB)/user-contrib/$(INSTALLDEFAULTROOT)/$$i`; \
	 install $$i $(COQLIB)/user-contrib/$(INSTALLDEFAULTROOT)/$$i; \
	 done)

clean:
	rm -f $(CMOFILES) $(CMIFILES) $(CMXFILES) $(CMXSFILES) $(OFILES) $(VOFILES) $(VIFILES) $(GFILES) $(MLFILES:.ml=.cmo) $(MLFILES:.ml=.cmx) *~
	rm -f all.ps all-gal.ps all.pdf all-gal.pdf all.glob $(VFILES:.v=.glob) $(HTMLFILES) $(GHTMLFILES) $(VFILES:.v=.tex) $(VFILES:.v=.g.tex) $(VFILES:.v=.v.d)
	- rm -rf html

archclean:
	rm -f *.cmx *.o


printenv: 
	@echo CAMLC =	$(CAMLC)
	@echo CAMLOPTC =	$(CAMLOPTC)
	@echo CAMLP4LIB =	$(CAMLP4LIB)

-include $(VFILES:.v=.v.d)
.SECONDARY: $(VFILES:.v=.v.d)

# WARNING
#
# This Makefile has been automagically generated
# Edit at your own risks !
#
# END OF WARNING



==> slamjs/coq-if/Makefile <==
#############################################################################
##  v      #                   The Coq Proof Assistant                     ##
## <O___,, #                INRIA - CNRS - LIX - LRI - PPS                 ##
##   \VV/  #                                                               ##
##    //   #  Makefile automagically generated by coq_makefile V8.3pl3     ##
#############################################################################

# WARNING
#
# This Makefile has been automagically generated
# Edit at your own risks !
#
# END OF WARNING

#
# This Makefile was generated by the command line :
# coq_makefile lib.v lambdajs.v simple_cfa.v cfa.v 
#

# 
# This Makefile may take 3 arguments passed as environment variables:
#   - COQBIN to specify the directory where Coq binaries resides;
#   - CAMLBIN and CAMLP4BIN to give the path for the OCaml and Camlp4/5 binaries.
COQLIB:=$(shell $(COQBIN)coqtop -where | sed -e 's/\\/\\\\/g')
CAMLP4:="$(shell $(COQBIN)coqtop -config | awk -F = '/CAMLP4=/{print $$2}')"
ifndef CAMLP4BIN
  CAMLP4BIN:=$(CAMLBIN)
endif

CAMLP4LIB:=$(shell $(CAMLP4BIN)$(CAMLP4) -where)

##########################
#                        #
# Libraries definitions. #
#                        #
##########################

OCAMLLIBS:=-I .
COQSRCLIBS:=-I $(COQLIB)/kernel -I $(COQLIB)/lib \
  -I $(COQLIB)/library -I $(COQLIB)/parsing \
  -I $(COQLIB)/pretyping -I $(COQLIB)/interp \
  -I $(COQLIB)/proofs -I $(COQLIB)/tactics \
  -I $(COQLIB)/toplevel \
  -I $(COQLIB)/plugins/cc \
  -I $(COQLIB)/plugins/dp \
  -I $(COQLIB)/plugins/extraction \
  -I $(COQLIB)/plugins/field \
  -I $(COQLIB)/plugins/firstorder \
  -I $(COQLIB)/plugins/fourier \
  -I $(COQLIB)/plugins/funind \
  -I $(COQLIB)/plugins/groebner \
  -I $(COQLIB)/plugins/interface \
  -I $(COQLIB)/plugins/micromega \
  -I $(COQLIB)/plugins/nsatz \
  -I $(COQLIB)/plugins/omega \
  -I $(COQLIB)/plugins/quote \
  -I $(COQLIB)/plugins/ring \
  -I $(COQLIB)/plugins/romega \
  -I $(COQLIB)/plugins/rtauto \
  -I $(COQLIB)/plugins/setoid_ring \
  -I $(COQLIB)/plugins/subtac \
  -I $(COQLIB)/plugins/subtac/test \
  -I $(COQLIB)/plugins/syntax \
  -I $(COQLIB)/plugins/xml
COQLIBS:=-I . 
COQDOCLIBS:=

##########################
#                        #
# Variables definitions. #
#                        #
##########################

ZFLAGS=$(OCAMLLIBS) $(COQSRCLIBS) -I $(CAMLP4LIB)
OPT:=
COQFLAGS:=-q $(OPT) $(COQLIBS) $(OTHERFLAGS) $(COQ_XML)
ifdef CAMLBIN
  COQMKTOPFLAGS:=-camlbin $(CAMLBIN) -camlp4bin $(CAMLP4BIN)
endif
COQC:=$(COQBIN)coqc
COQDEP:=$(COQBIN)coqdep -c
GALLINA:=$(COQBIN)gallina
COQDOC:=$(COQBIN)coqdoc
COQMKTOP:=$(COQBIN)coqmktop
CAMLLIB:=$(shell $(CAMLBIN)ocamlc.opt -where)
CAMLC:=$(CAMLBIN)ocamlc.opt -c -rectypes
CAMLOPTC:=$(CAMLBIN)ocamlopt.opt -c -rectypes
CAMLLINK:=$(CAMLBIN)ocamlc.opt -rectypes
CAMLOPTLINK:=$(CAMLBIN)ocamlopt.opt -rectypes
GRAMMARS:=grammar.cma
CAMLP4EXTEND:=pa_extend.cmo pa_macro.cmo q_MLast.cmo
CAMLP4OPTIONS:=
PP:=-pp "$(CAMLP4BIN)$(CAMLP4)o -I $(CAMLLIB) -I . $(COQSRCLIBS) $(CAMLP4EXTEND) $(GRAMMARS) $(CAMLP4OPTIONS) -impl"

###################################
#                                 #
# Definition of the "all" target. #
#                                 #
###################################

VFILES:=lib.v\
  lambdajs.v\
  simple_cfa.v\
  cfa.v
VOFILES:=$(VFILES:.v=.vo)
VOFILES0:=$(filter-out ,$(VOFILES))
GLOBFILES:=$(VFILES:.v=.glob)
VIFILES:=$(VFILES:.v=.vi)
GFILES:=$(VFILES:.v=.g)
HTMLFILES:=$(VFILES:.v=.html)
GHTMLFILES:=$(VFILES:.v=.g.html)

all: $(VOFILES) 
spec: $(VIFILES)

gallina: $(GFILES)

html: $(GLOBFILES) $(VFILES)
	- mkdir -p html
	$(COQDOC) -toc -html $(COQDOCLIBS) -d html $(VFILES)

gallinahtml: $(GLOBFILES) $(VFILES)
	- mkdir -p html
	$(COQDOC) -toc -html -g $(COQDOCLIBS) -d html $(VFILES)

all.ps: $(VFILES)
	$(COQDOC) -toc -ps $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.ps: $(VFILES)
	$(COQDOC) -toc -ps -g $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all.pdf: $(VFILES)
	$(COQDOC) -toc -pdf $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`

all-gal.pdf: $(VFILES)
	$(COQDOC) -toc -pdf -g $(COQDOCLIBS) -o $@ `$(COQDEP) -sort -suffix .v $(VFILES)`



####################
#                  #
# Special targets. #
#                  #
####################

.PHONY: all opt byte archclean clean install depend html

%.vo %.glob: %.v
	$(COQC) $(COQDEBUG) $(COQFLAGS) $*

%.vi: %.v
	$(COQC) -i $(COQDEBUG) $(COQFLAGS) $*

%.g: %.v
	$(GALLINA) $<

%.tex: %.v
	$(COQDOC) -latex $< -o $@

%.html: %.v %.glob
	$(COQDOC) -html $< -o $@

%.g.tex: %.v
	$(COQDOC) -latex -g $< -o $@

%.g.html: %.v %.glob
	$(COQDOC) -html -g $< -o $@

%.v.d: %.v
	$(COQDEP) -slash $(COQLIBS) "$<" > "$@" || ( RV=$$?; rm -f "$@"; exit $${RV} )

byte:
	$(MAKE) all "OPT:=-byte"

opt:
	$(MAKE) all "OPT:=-opt"

install:
	mkdir -p $(COQLIB)/user-contrib
	(for i in $(VOFILES0); do \
	 install -d `dirname $(COQLIB)/user-contrib/$(INSTALLDEFAULTROOT)/$$i`; \
	 install $$i $(COQLIB)/user-contrib/$(INSTALLDEFAULTROOT)/$$i; \
	 done)

clean:
	rm -f $(CMOFILES) $(CMIFILES) $(CMXFILES) $(CMXSFILES) $(OFILES) $(VOFILES) $(VIFILES) $(GFILES) $(MLFILES:.ml=.cmo) $(MLFILES:.ml=.cmx) *~
	rm -f all.ps all-gal.ps all.pdf all-gal.pdf all.glob $(VFILES:.v=.glob) $(HTMLFILES) $(GHTMLFILES) $(VFILES:.v=.tex) $(VFILES:.v=.g.tex) $(VFILES:.v=.v.d)
	- rm -rf html

archclean:
	rm -f *.cmx *.o


printenv: 
	@echo CAMLC =	$(CAMLC)
	@echo CAMLOPTC =	$(CAMLOPTC)
	@echo CAMLP4LIB =	$(CAMLP4LIB)

-include $(VFILES:.v=.v.d)
.SECONDARY: $(VFILES:.v=.v.d)

# WARNING
#
# This Makefile has been automagically generated
# Edit at your own risks !
#
# END OF WARNING


